Two-dimensional distributed-phase-reference protocol for quantum key distribution

Quantum key distribution (QKD) and quantum communication enable the secure exchange of information between remote parties. Currently, the distributed-phase-reference (DPR) protocols, which are based on weak coherent pulses, are among the most practical solutions for long-range QKD. During the last 10 years, long-distance fiber-based DPR systems have been successfully demonstrated, although fundamental obstacles such as intrinsic channel losses limit their performance. Here, we introduce the first two-dimensional DPR-QKD protocol in which information is encoded in the time and phase of weak coherent pulses. The ability of extracting two bits of information per detection event, enables a higher secret key rate in specific realistic network scenarios. Moreover, despite the use of more dimensions, the proposed protocol remains simple, practical, and fully integrable.

==> preamble.tex <==
%\documentclass[10pt,a4paper,twocolumn]{article}

%\usepackage{siunitx}
%\usepackage{float}
%\usepackage{tikz}
%\usepackage{xcolor}
%\usepackage{transparent}

\usepackage{braket}
\usepackage{nicefrac}

%\usepackage[english]{babel} 
%\usepackage[top=2.8cm,bottom=2.8cm,left=2.cm,right=2.cm]{geometry}  % ændre margen 
%\usepackage{amsmath,amsfonts,amssymb}  % matematiske tegn og symboler
% \usepackage{mathpazo}
% \linespread{1.05}
\usepackage{graphicx,subfigure}  % billeder kan lægges ind
%\graphicspath{{./Figures/}{./PSTricks/}}  % billeder kan lægges i undermappen "billeder"
%\pagestyle{plain}
%\usepackage{multirow}
%\usepackage{appendix}
%\usepackage{wrapfig}

%\usepackage{setspace}

%it was biblio style numeric-comp

%\usepackage{csquotes}
%\usepackage[bibstyle=ieee,
%citestyle=numeric-comp, 
%hyperref,sorting=none,backend=biber,doi=false,isbn=false,url=false,firstinits=true,uniquename=init,maxcitenames=4,maxbibnames=3,minbibnames=3]{biblatex}
%\bibliography{Mendeley.bib}
%\AtEveryBibitem{\clearfield{pages}}
%\AtEveryBibitem{\clearfield{month}}
%\renewbibmacro{in:}{}

%\DeclareFieldFormat
%[article,inbook,incollection,inproceedings,patent,thesis,unpublished]
%{title}{#1\isdot}


%\usepackage{enumitem}
%\usepackage{caption3} % load caption package kernel first
%\DeclareCaptionOption{parskip}[]{} % disable "parskip" caption option
%\usepackage[font=small,labelfont=bf]{caption}
%\usepackage[final]{pdfpages}
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage{tikz}
%\usepackage{sidecap}
%\sidecaptionvpos{figure}{t}
%\setlength{\parskip}{1ex plus 0.5ex minus 0.2ex}
%\setlength{\parindent}{4mm}


%\newcommand{\red}{\color{red}}
%\newcommand{\green}{\color{green}}
%\newcommand{\blue}{\color{blue}}



%\usepackage[pdftex]{hyperref} 

